Approximating High-Dimensional Minimal Surfaces with Physics-Informed Neural Networks

In this paper, we compute numerical approximations of the minimal surfaces, an essential type of Partial Differential Equation (PDE), in higher dimensions. Classical methods cannot handle it in this case because of the Curse of Dimensionality, where the computational cost of these methods increases exponentially fast in response to higher problem dimensions, far beyond the computing capacity of any modern supercomputers. Only in the past few years have machine learning researchers been able to mitigate this problem. The solution method chosen here is a model known as a Physics-Informed Neural Network (PINN) which trains a deep neural network (DNN) to solve the minimal surface PDE. It can be scaled up into higher dimensions and trained relatively quickly even on a laptop with no GPU. Due to the inability to view the high-dimension output, our data is presented as snippets of a higher-dimension shape with enough fixed axes so that it is viewable with 3-D graphs. Not only will the functionality of this method be tested, but we will also explore potential limitations in the method's performance.

==> cover_letter.tex <==
Dear Editor and Anonymous Reviewers,

We are writing to submit our work “Approximating High-Dimensional Minimal Surfaces with Physics-Informed Neural Networks” to Involve. In this work, we developed a computational method to solve the minimal surface problem defined in potentially high dimensional spaces. We parameterized the solution as a deep neural network and convert the minimal surface problem into an optimization problem of the network parameters based on the partial differential equation formulation of the former. Our problem setting and actual computations do not need spatial discretization nor basis representations and is a promising approach to solve minimal surface problems in high dimension.

The author Steven Zhou is currently a 12th grade high school student at the Gwinnett School of Mathematics, Science, and Technology (GSMST), Lawrenceville, Georgia, USA. This work, including the problem setting, numerical implementations, and manuscript drafting, is done by Mr. Zhou under the supervision of the coauthor, Dr. Xiaojing Ye, who is an associate professor of mathematics at Georgia State University, Atlanta, Georgia, USA. This work is not published or currently under review by any other journal or conference.

We attest that at least one-third of the authors of this paper are high-school, undergraduate or graduate students.

We appreciate any of your comments on our work. If you have further questions, please do not hesitate to contact us.

Best regards,
Steven and Xiaojing

Potential reviewers:

Dr. Christina Frederick
Associate Professor, Mathematical Sciences, New Jersey Institute of Technology, Newark, New Jersey, USA
Email: christin@njit.edu

Dr. Rongjie Lai
Professor, Department of Mathematics, Purdue University, West Lafayette, Indiana, USA
lairj@purdue.edu

Dr. Wuchen Li
Assistant Professor, Department of Mathematics, University of South Carolina, Columbia, South Carolina, USA
Email: wuchen@mailbox.sc.edu

Dr. Wei Zhu
Professor, Department of Mathematics, The University of Alabama, Tuscaloosa, AL 35487, USA
Email: wzhu7@ua.edu


